Choices, intervals and equidistribution

We give a sufficient condition for a random sequence in [0,1] generated by a $\Psi$-process to be equidistributed. The condition is met by the canonical example -- the $\max$-2 process -- where the $n$th term is whichever of two uniformly placed points falls in the larger gap formed by the previous $n-1$ points. This solves an open problem from Itai Benjamini, Pascal Maillard and Elliot Paquette. We also deduce equidistribution for more general $\Psi$-processes. This includes an interpolation of the $\min$-2 and $\max$-2 processes that is biased towards $\min$-2.

==> figures5.tex <==

\begin{center}
\begin{figure} \label{fig:1}
\begin{tikzpicture}
\node[label=left:\rotatebox{90}{Density}] at (-8.5,4) {};
\node at (-3.1,0.5) {Position};
\node[blue, right] at (-8.1,1.35){$\max$-2};
\node[green, right] at (-8.1,3.25){uniform};
\node[right] at (-8.1,5.2){$20\%$-min-2};

\begin{scope}[shift={(-8cm,4.955)}]

\begin{groupplot}[
group style={
group size=2 by 3,
xticklabels at=edge bottom,
vertical sep=0pt,
horizontal sep = .9 cm,
xlabels at=edge bottom,
ylabels at=edge left
},
width=6cm,
xmin = 0, xmax = 1,
%xtick = {0,.2,.4,.6,.8,1}
%ylabel=Density
]

\nextgroupplot[ymin=0.6,ymax=1.4,
    xtick={1},
	ytick={3},
%	axis y discontinuity=crunch,
	height=3.5 cm, yticklabel pos=right
	]
		\addplot[black, dashed, mark size = 0, mark = *] table {
		0 1.2
		1 1.2
		 };
		 		\addplot[black, dashed, mark size = 0, mark = *] table {
		0 .8
		1 .8
		 };
	\addplot[black, thick, mark size = 0, mark = *] table {
0.0 0.930000000000000
0.01 1.00000000000000
0.02 1.33000000000000
0.03 1.14000000000000
0.04 1.06000000000000
0.05 0.910000000000000
0.06 1.02000000000000
0.07 0.980000000000000
0.08 1.02000000000000
0.09 0.950000000000000
0.1 1.32000000000000
0.11 1.18000000000000
0.12 0.890000000000000
0.13 1.07000000000000
0.14 1.09000000000000
0.15 0.780000000000000
0.16 0.960000000000000
0.17 1.12000000000000
0.18 1.02000000000000
0.19 1.17000000000000
0.2 1.31000000000000
0.21 1.21000000000000
0.22 0.820000000000000
0.23 0.920000000000000
0.24 1.02000000000000
0.25 0.950000000000000
0.26 0.920000000000000
0.27 0.970000000000000
0.28 1.01000000000000
0.29 1.12000000000000
0.3 1.20000000000000
0.31 0.780000000000000
0.32 0.920000000000000
0.33 0.920000000000000
0.34 1.28000000000000
0.35 0.850000000000000
0.36 0.840000000000000
0.37 1.07000000000000
0.38 1.35000000000000
0.39 1.00000000000000
0.4 0.950000000000000
0.41 1.09000000000000
0.42 1.15000000000000
0.43 1.23000000000000
0.44 0.950000000000000
0.45 1.13000000000000
0.46 1.10000000000000
0.47 0.900000000000000
0.48 0.910000000000000
0.49 0.910000000000000
0.5 0.980000000000000
0.51 0.810000000000000
0.52 1.31000000000000
0.53 0.790000000000000
0.54 1.09000000000000
0.55 1.13000000000000
0.56 0.950000000000000
0.57 1.19000000000000
0.58 0.980000000000000
0.59 0.650000000000000
0.6 0.820000000000000
0.61 1.00000000000000
0.62 1.15000000000000
0.63 1.20000000000000
0.64 0.810000000000000
0.65 0.790000000000000
0.66 1.00000000000000
0.67 0.910000000000000
0.68 1.05000000000000
0.69 0.890000000000000
0.7 0.850000000000000
0.71 0.980000000000000
0.72 1.09000000000000
0.73 1.20000000000000
0.74 0.770000000000000
0.75 1.15000000000000
0.76 1.08000000000000
0.77 1.13000000000000
0.78 0.780000000000000
0.79 1.08000000000000
0.8 0.850000000000000
0.81 0.950000000000000
0.82 0.940000000000000
0.83 0.990000000000000
0.84 1.00000000000000
0.85 1.05000000000000
0.86 1.15000000000000
0.87 1.05000000000000
0.88 0.710000000000000
0.89 1.04000000000000
0.9 1.10000000000000
0.91 0.960000000000000
0.92 1.00000000000000
0.93 0.970000000000000
0.94 1.00000000000000
0.95 0.820000000000000
0.96 1.09000000000000
0.97 1.04000000000000
0.98 1.08000000000000
1 1.05
};]



\nextgroupplot[ymin=0.6,ymax=1.4,
    xtick={1},
	ytick={3},
%	axis y discontinuity=crunch,
	height=3.5 cm, yticklabel pos=right
	]
		\addplot[black, dashed, mark size = 0, mark = *] table {
		0 1.2
		1 1.2
		 };
		 		\addplot[black, dashed, mark size = 0, mark = *] table {
		0 .8
		1 .8
		 };
	\addplot[black, thick, mark size = 0, mark = *] table { 
0.0 1.01000000000000
0.01 1.02000000000000
0.02 1.01000000000000
0.03 1.02000000000000
0.04 1.01000000000000
0.05 1.00000000000000
0.06 1.00000000000000
0.07 0.990000000000000
0.08 1.01000000000000
0.09 1.02000000000000
0.1 1.02000000000000
0.11 0.990000000000000
0.12 1.01000000000000
0.13 1.01000000000000
0.14 1.03000000000000
0.15 0.990000000000000
0.16 1.01000000000000
0.17 1.02000000000000
0.18 1.02000000000000
0.19 1.02000000000000
0.2 1.01000000000000
0.21 1.00000000000000
0.22 1.03000000000000
0.23 1.01000000000000
0.24 1.00000000000000
0.25 1.03000000000000
0.26 1.02000000000000
0.27 1.01000000000000
0.28 1.01000000000000
0.29 1.02000000000000
0.3 1.02000000000000
0.31 1.02000000000000
0.32 1.02000000000000
0.33 0.980000000000000
0.34 1.02000000000000
0.35 1.00000000000000
0.36 1.01000000000000
0.37 0.990000000000000
0.38 1.01000000000000
0.39 1.02000000000000
0.4 0.990000000000000
0.41 1.03000000000000
0.42 1.00000000000000
0.43 0.980000000000000
0.44 1.00000000000000
0.45 1.01000000000000
0.46 0.980000000000000
0.47 1.04000000000000
0.48 0.980000000000000
0.49 1.00000000000000
0.5 1.01000000000000
0.51 1.02000000000000
0.52 1.00000000000000
0.53 1.02000000000000
0.54 1.02000000000000
0.55 1.01000000000000
0.56 1.00000000000000
0.57 1.02000000000000
0.58 0.990000000000000
0.59 1.02000000000000
0.6 1.01000000000000
0.61 1.00000000000000
0.62 1.02000000000000
0.63 1.01000000000000
0.64 0.990000000000000
0.65 1.02000000000000
0.66 1.03000000000000
0.67 1.00000000000000
0.68 1.00000000000000
0.69 1.02000000000000
0.7 1.01000000000000
0.71 1.01000000000000
0.72 1.01000000000000
0.73 1.00000000000000
0.74 1.00000000000000
0.75 1.01000000000000
0.76 1.00000000000000
0.77 1.00000000000000
0.78 1.01000000000000
0.79 1.01000000000000
0.8 1.02000000000000
0.81 1.01000000000000
0.82 1.00000000000000
0.83 1.03000000000000
0.84 1.02000000000000
0.85 1.00000000000000
0.86 1.02000000000000
0.87 1.01000000000000
0.88 1.01000000000000
0.89 1.02000000000000
0.9 1.01000000000000
0.91 1.01000000000000
0.92 1.01000000000000
0.93 1.01000000000000
0.94 1.03000000000000
0.95 1.02000000000000
0.96 1.00000000000000
0.97 1.02000000000000
0.98 1.02000000000000
.99 1.0
1. .98
	};
	]


\nextgroupplot[ymin=0.6,ymax=1.4,
	ytick={.8,1.2},
	xtick = {1},
%	axis y discontinuity=crunch,
	yticklabel pos=left,
	height=3.5 cm,
%	xlabel=Position,
	]
	\addplot[black, dashed, mark size = 0, mark = *] table {
		0 1.2
		1 1.2
		 };
		 		\addplot[black, dashed, mark size = 0, mark = *] table {
		0 .8
		1 .8
		 };
	
	\addplot[green, thick, mark size = 0, mark = square*] table {
0.0 1.01000000000000
0.01 1.11000000000000
0.02 0.960000000000000
0.03 0.820000000000000
0.04 1.02000000000000
0.05 1.10000000000000
0.06 0.980000000000000
0.07 1.08000000000000
0.08 1.10000000000000
0.09 1.09000000000000
0.1 1.00000000000000
0.11 1.01000000000000
0.12 1.08000000000000
0.13 0.980000000000000
0.14 1.05000000000000
0.15 1.02000000000000
0.16 1.12000000000000
0.17 1.06000000000000
0.18 1.17000000000000
0.19 0.920000000000000
0.2 0.880000000000000
0.21 1.05000000000000
0.22 0.780000000000000
0.23 0.900000000000000
0.24 0.950000000000000
0.25 1.06000000000000
0.26 1.00000000000000
0.27 0.940000000000000
0.28 1.01000000000000
0.29 1.13000000000000
0.3 0.940000000000000
0.31 1.12000000000000
0.32 1.12000000000000
0.33 0.880000000000000
0.34 0.940000000000000
0.35 0.990000000000000
0.36 0.850000000000000
0.37 1.12000000000000
0.38 1.02000000000000
0.39 1.06000000000000
0.4 1.02000000000000
0.41 1.08000000000000
0.42 0.860000000000000
0.43 1.05000000000000
0.44 1.01000000000000
0.45 1.03000000000000
0.46 0.820000000000000
0.47 1.16000000000000
0.48 1.03000000000000
0.49 1.08000000000000
0.5 0.850000000000000
0.51 1.08000000000000
0.52 0.850000000000000
0.53 0.930000000000000
0.54 0.990000000000000
0.55 0.890000000000000
0.56 1.06000000000000
0.57 1.05000000000000
0.58 0.920000000000000
0.59 0.950000000000000
0.6 0.920000000000000
0.61 0.950000000000000
0.62 1.23000000000000
0.63 0.960000000000000
0.64 0.960000000000000
0.65 0.870000000000000
0.66 0.940000000000000
0.67 1.11000000000000
0.68 1.04000000000000
0.69 1.03000000000000
0.7 1.00000000000000
0.71 1.15000000000000
0.72 0.940000000000000
0.73 1.03000000000000
0.74 0.870000000000000
0.75 1.00000000000000
0.76 1.13000000000000
0.77 0.920000000000000
0.78 1.00000000000000
0.79 1.14000000000000
0.8 1.18000000000000
0.81 0.990000000000000
0.82 1.02000000000000
0.83 0.990000000000000
0.84 1.06000000000000
0.85 1.15000000000000
0.86 1.03000000000000
0.87 1.00000000000000
0.88 1.05000000000000
0.89 0.930000000000000
0.9 1.14000000000000
0.91 0.970000000000000
0.92 0.960000000000000
0.93 1.24000000000000
0.94 1.08000000000000
0.95 1.03000000000000
0.96 1.07000000000000
0.97 0.900000000000000
0.98 1.01000000000000
1 1
};]

\nextgroupplot[ymin=0.6,ymax=1.4,
	ytick={3},
	xtick = {1},
%	axis y discontinuity=crunch,
	yticklabel pos=left,
	height=3.5 cm,
%	xlabel=Position,
	]
	\addplot[black, dashed, mark size = 0, mark = *] table {
		0 1.2
		1 1.2
		 };
		 		\addplot[black, dashed, mark size = 0, mark = *] table {
		0 .8
		1 .8
		 };
	
	\addplot[green, thick, mark size = 0, mark = square*] table {
       	
0.0 1.01000000000000
0.01 1.01000000000000
0.02 0.990000000000000
0.03 1.02000000000000
0.04 1.02000000000000
0.05 1.00000000000000
0.06 1.02000000000000
0.07 1.01000000000000
0.08 1.02000000000000
0.09 1.01000000000000
0.1 1.02000000000000
0.11 1.01000000000000
0.12 1.02000000000000
0.13 1.01000000000000
0.14 1.01000000000000
0.15 0.990000000000000
0.16 1.00000000000000
0.17 1.00000000000000
0.18 1.01000000000000
0.19 1.01000000000000
0.2 1.01000000000000
0.21 1.01000000000000
0.22 1.01000000000000
0.23 1.00000000000000
0.24 1.03000000000000
0.25 1.01000000000000
0.26 1.01000000000000
0.27 1.04000000000000
0.28 1.00000000000000
0.29 1.00000000000000
0.3 1.01000000000000
0.31 1.02000000000000
0.32 1.02000000000000
0.33 1.02000000000000
0.34 1.01000000000000
0.35 1.00000000000000
0.36 1.02000000000000
0.37 1.02000000000000
0.38 1.00000000000000
0.39 1.01000000000000
0.4 1.03000000000000
0.41 0.990000000000000
0.42 1.01000000000000
0.43 0.980000000000000
0.44 0.990000000000000
0.45 1.03000000000000
0.46 0.990000000000000
0.47 0.990000000000000
0.48 1.00000000000000
0.49 1.01000000000000
0.5 1.00000000000000
0.51 1.02000000000000
0.52 1.00000000000000
0.53 0.990000000000000
0.54 1.02000000000000
0.55 0.990000000000000
0.56 1.01000000000000
0.57 1.00000000000000
0.58 1.02000000000000
0.59 1.00000000000000
0.6 1.03000000000000
0.61 1.01000000000000
0.62 1.00000000000000
0.63 1.00000000000000
0.64 1.02000000000000
0.65 1.02000000000000
0.66 1.00000000000000
0.67 1.01000000000000
0.68 1.02000000000000
0.69 1.02000000000000
0.7 1.02000000000000
0.71 1.01000000000000
0.72 1.02000000000000
0.73 1.01000000000000
0.74 1.01000000000000
0.75 1.01000000000000
0.76 1.02000000000000
0.77 1.02000000000000
0.78 1.00000000000000
0.79 1.01000000000000
0.8 1.01000000000000
0.81 1.02000000000000
0.82 1.01000000000000
0.83 1.01000000000000
0.84 1.00000000000000
0.85 1.02000000000000
0.86 1.01000000000000
0.87 0.980000000000000
0.88 1.02000000000000
0.89 1.00000000000000
0.9 1.02000000000000
0.91 1.02000000000000
0.92 1.01000000000000
0.93 1.00000000000000
0.94 1.03000000000000
0.95 1.01000000000000
0.96 1.01000000000000
0.97 1.02000000000000
0.98 1.04000000000000
1 1
};]



\nextgroupplot[ymin=0.6,ymax=1.4,
	ytick={3},
	xtick = {0,1},
	%axis y discontinuity=crunch,
	yticklabel pos=right,
	height=3.5cm,
%	xlabel=Position,
	]
	
	\addplot[black, dashed, mark size = 0, mark = *] table {
		0 1.2
		1 1.2
		 };
		 		\addplot[black, dashed, mark size = 0, mark = *] table {
		0 .8
		1 .8
		 };
\addplot[blue, thick] table {
0.0 1.08000000000000
0.01 1.02000000000000
0.02 0.950000000000000
0.03 0.910000000000000
0.04 0.980000000000000
0.05 0.930000000000000
0.06 1.05000000000000
0.07 0.870000000000000
0.08 1.12000000000000
0.09 1.05000000000000
0.1 0.860000000000000
0.11 0.950000000000000
0.12 1.02000000000000
0.13 0.950000000000000
0.14 1.07000000000000
0.15 0.900000000000000
0.16 1.11000000000000
0.17 0.970000000000000
0.18 1.03000000000000
0.19 1.02000000000000
0.2 1.02000000000000
0.21 1.01000000000000
0.22 0.990000000000000
0.23 1.12000000000000
0.24 0.970000000000000
0.25 1.01000000000000
0.26 1.02000000000000
0.27 0.940000000000000
0.28 1.06000000000000
0.29 1.03000000000000
0.3 1.01000000000000
0.31 0.950000000000000
0.32 1.03000000000000
0.33 1.01000000000000
0.34 0.950000000000000
0.35 0.960000000000000
0.36 1.08000000000000
0.37 1.10000000000000
0.38 1.00000000000000
0.39 0.950000000000000
0.4 1.02000000000000
0.41 0.960000000000000
0.42 1.03000000000000
0.43 1.05000000000000
0.44 1.06000000000000
0.45 0.960000000000000
0.46 1.07000000000000
0.47 1.05000000000000
0.48 1.03000000000000
0.49 1.03000000000000
0.5 1.09000000000000
0.51 1.00000000000000
0.52 1.11000000000000
0.53 0.950000000000000
0.54 0.970000000000000
0.55 1.09000000000000
0.56 1.03000000000000
0.57 0.970000000000000
0.58 1.10000000000000
0.59 1.00000000000000
0.6 1.06000000000000
0.61 1.06000000000000
0.62 0.990000000000000
0.63 0.980000000000000
0.64 0.980000000000000
0.65 1.15000000000000
0.66 1.01000000000000
0.67 0.950000000000000
0.68 1.03000000000000
0.69 1.04000000000000
0.7 1.03000000000000
0.71 1.01000000000000
0.72 1.14000000000000
0.73 0.930000000000000
0.74 0.910000000000000
0.75 0.990000000000000
0.76 1.06000000000000
0.77 1.05000000000000
0.78 1.01000000000000
0.79 0.990000000000000
0.8 0.980000000000000
0.81 1.09000000000000
0.82 1.00000000000000
0.83 1.01000000000000
0.84 1.08000000000000
0.85 1.15000000000000
0.86 0.900000000000000
0.87 0.980000000000000
0.88 0.880000000000000
0.89 1.09000000000000
0.9 1.09000000000000
0.91 0.960000000000000
0.92 1.00000000000000
0.93 1.09000000000000
0.94 0.970000000000000
0.95 0.990000000000000
0.96 0.990000000000000
0.97 0.890000000000000
0.98 0.990000000000000
1 1
};]

\nextgroupplot[ymin=0.6,ymax=1.4,
	ytick={3},
	xtick = {0,1},
	%axis y discontinuity=crunch,
	yticklabel pos=right,
	height=3.5cm,
%	xlabel=Position,
	]
	
	\addplot[black, dashed, mark size = 0, mark = *] table {
		0 1.2
		1 1.2
		 };
		 		\addplot[black, dashed, mark size = 0, mark = *] table {
		0 .8
		1 .8
		 };
\addplot[blue, thick] table {
0.0 1.01000000000000
0.01 1.01000000000000
0.02 1.01000000000000
0.03 1.01000000000000
0.04 1.00000000000000
0.05 1.00000000000000
0.06 1.01000000000000
0.07 1.01000000000000
0.08 1.01000000000000
0.09 1.01000000000000
0.1 1.01000000000000
0.11 1.01000000000000
0.12 1.01000000000000
0.13 1.01000000000000
0.14 1.01000000000000
0.15 1.01000000000000
0.16 1.02000000000000
0.17 1.01000000000000
0.18 1.00000000000000
0.19 1.02000000000000
0.2 1.00000000000000
0.21 1.00000000000000
0.22 1.02000000000000
0.23 1.01000000000000
0.24 1.01000000000000
0.25 1.01000000000000
0.26 1.01000000000000
0.27 1.01000000000000
0.28 1.00000000000000
0.29 1.01000000000000
0.3 1.00000000000000
0.31 1.01000000000000
0.32 1.01000000000000
0.33 1.02000000000000
0.34 1.01000000000000
0.35 1.02000000000000
0.36 1.01000000000000
0.37 1.00000000000000
0.38 1.01000000000000
0.39 1.02000000000000
0.4 1.01000000000000
0.41 1.00000000000000
0.42 1.01000000000000
0.43 1.03000000000000
0.44 1.01000000000000
0.45 1.02000000000000
0.46 1.01000000000000
0.47 1.01000000000000
0.48 1.02000000000000
0.49 1.00000000000000
0.5 1.01000000000000
0.51 1.01000000000000
0.52 1.02000000000000
0.53 1.01000000000000
0.54 1.00000000000000
0.55 1.01000000000000
0.56 1.00000000000000
0.57 1.02000000000000
0.58 1.01000000000000
0.59 1.02000000000000
0.6 1.01000000000000
0.61 1.01000000000000
0.62 1.01000000000000
0.63 1.02000000000000
0.64 1.01000000000000
0.65 1.01000000000000
0.66 1.02000000000000
0.67 1.00000000000000
0.68 1.01000000000000
0.69 1.01000000000000
0.7 1.03000000000000
0.71 1.01000000000000
0.72 1.01000000000000
0.73 1.01000000000000
0.74 1.01000000000000
0.75 1.01000000000000
0.76 1.00000000000000
0.77 1.01000000000000
0.78 1.00000000000000
0.79 1.02000000000000
0.8 1.01000000000000
0.81 1.00000000000000
0.82 1.00000000000000
0.83 0.990000000000000
0.84 1.02000000000000
0.85 1.01000000000000
0.86 1.01000000000000
0.87 1.01000000000000
0.88 1.01000000000000
0.89 1.01000000000000
0.9 1.00000000000000
0.91 1.02000000000000
0.92 1.02000000000000
0.93 1.01000000000000
0.94 1.02000000000000
0.95 1.01000000000000
0.96 1.02000000000000
0.97 1.02000000000000
0.98 1.00000000000000
1 1
};]








\end{groupplot}

\end{scope}

%\begin{scope}[shift={(-3cm,0)}]
%
%\begin{axis}[xlabel = {$\%\min$-2}, ylabel = {Std. deviation}, height = 9cm , width = 6 cm , xtick = {0,.5,.6}, ytick = {.12, .14, .16}, ymax = .165, ymin = .112, ytick pos = right]
% \addplot[only marks, color = green, mark size= 3pt] 
%        table[x index=0, y index = 1] {
%        .495 .1399
%        };
% \addplot[only marks, color = black, mark size= 3pt] 
%        table[x index=0, y index = 1] {
%        0.6 0.155940000000000
%                };
% \addplot[only marks, color = blue, mark size= 3pt] 
%        table[x index=0, y index = 1] {
%        .0 .11813
%        };
%
%     \addplot[very thick, color = black, mark size= 0pt, xtick = {0,.5,.6,1}] 
%        table[x index=0, y index = 1] {
%0.0 0.118130000000000
%0.02 0.117500000000000
%0.04 0.117450000000000
%0.06 0.118650000000000
%0.08 0.120910000000000
%0.1 0.119720000000000
%0.12 0.121660000000000
%0.14 0.121750000000000
%0.16 0.123770000000000
%0.18 0.122640000000000
%0.2 0.121850000000000
%0.22 0.120650000000000
%0.24 0.125110000000000
%0.26 0.122190000000000
%0.28 0.125840000000000
%0.3 0.128540000000000
%0.32 0.128940000000000
%0.34 0.131060000000000
%0.36 0.130670000000000
%0.38 0.129890000000000
%0.4 0.130720000000000
%0.42 0.130340000000000
%0.44 0.136920000000000
%0.46 0.133970000000000
%0.48 0.138330000000000
%0.5 0.142030000000000
%0.52 0.140990000000000
%0.54 0.144080000000000
%0.56 0.143580000000000
%0.58 0.151950000000000
%0.6 0.155940000000000
%        };
%\end{axis}
%\end{scope}
\end{tikzpicture}
\caption{The empirical density of $10^4$ (left) and $10^6$ (right) points for the $20\%$-$\min$-2/$80\%$-uniform mixture, the uniform process, and the $\max$-2 process. 
%Each is equidistributed by \thref{thm:main}. 
The interval is discretized into 100 equally sized bins. 
%The interval $[0,1]$ is discretized into 100 equal sized bins.
%
%On the right we see the standard deviation of the density increases as the $\min$-2 process becomes more prevalent in the blend. 
}
\end{figure}
\end{center}
